Scalable Interpretability via Polynomials

Generalized Additive Models (GAMs) have quickly become the leading choice for inherently-interpretable machine learning. However, unlike uninterpretable methods such as DNNs, they lack expressive power and easy scalability, and are hence not a feasible alternative for real-world tasks. We present a new class of GAMs that use tensor rank decompositions of polynomials to learn powerful, {\em inherently-interpretable} models. Our approach, titled Scalable Polynomial Additive Models (SPAM) is effortlessly scalable and models {\em all} higher-order feature interactions without a combinatorial parameter explosion. SPAM outperforms all current interpretable approaches, and matches DNN/XGBoost performance on a series of real-world benchmarks with up to hundreds of thousands of features. We demonstrate by human subject evaluations that SPAMs are demonstrably more interpretable in practice, and are hence an effortless replacement for DNNs for creating interpretable and high-performance systems suitable for large-scale machine learning. Source code is available at https://github.com/facebookresearch/nbm-spam.

==> NeurIPS2022_LowRankTensors (3)/sec/experiments_offline.tex <==
\section{Offline Experiments}
\label{sec:experiments}
Here we evaluate SPAM against a set of benchmark algorithms on both classification and regression problems. The baseline approaches we consider are (see Appendix Section~\ref{sec:appendix_experiment_details} for precise details):
\begin{itemize}[leftmargin=*,itemsep=0pt,topsep=0pt,parsep=0pt,partopsep=0pt]
    \item {\bf Deep Neural Networks (DNN)}: These are standard multi-layer fully-connected neural networks included to demonstrate an upper-bound on performance. These are explained via the perturbation-based LIME~\citep{ribeiro2016should} and SHAP~\citep{lundberg2017unified} methods in Section~\ref{sec:human_evaluations}.
    \item {\bf Linear / Logistic Regression}: These serve as our baseline interpretable models. We learn both $L_1$ and $L_2-$regularized models on unary and pairwise features (${d \choose 2}$ features) with minibatch SGD.
    \item {\bf Gradient Boosted Trees (XGBoost)}: We use the library {\tt xgboost}. This baseline is mainly to compare accuracy, as the number of trees required are typically large and are hence uninterpretable.
    \item {\bf Explainable Boosting Machines (EBMs)}~\citep{lou2013accurate}: EBMs use millions of shallow bagged trees operating on each feature at a time. Note that this approach is not scalable to datasets with many features or multi-class problems. We report scores on the datasets where we successfully trained EBMs without sophisticated engineering, using the {\sf interpretml} library~\citep{nori2019interpretml}.
    \item {\bf Neural Additive Models (NAMs)}~\citep{agarwal2021neural}: These models are neural network extensions of prior EBMs. Note that this method also does not scale to some datasets.
\end{itemize}

{\bf Training Setup}. SPAM is implemented by learning $L_1/L_2$-regularized variants by minibatch SGD implemented in PyTorch. For regression tasks, we measure the root mean squared error (RMSE). For binary classification, we report the area under the ROC (AUROC), for multi-class classification, we report the top-1 accuracy (Acc@1), and finally, for object detection, we report mean Average Precision (mAP). We tune hyperparameters via random sampling approach over a grid. Note that for all experiments, both NAM and {\sc SPAM-Neural} have identical MLP structures to ensure identical approximation power. For definitions of metrics and hyperparameter ranges, see Appendix Section~\ref{sec:appendix_experiment_details}.

\subsection{Measuring Benchmark Performance}
\setlength{\tabcolsep}{1.5pt}
\begin{table}[t]
\caption{Evaluation of SPAM on benchmarks against prior work. ($\uparrow$): higher is better, ($\downarrow$): lower is better, $^{**}$: variance across trials is $<0.001$, $^{*~}$: variance across trials is $<0.005$.  {\color{maroon}\bf Boldface red} denotes the best {\color{maroon}\bf black-box} model, {\color{OliveGreen}\bf boldface green} denotes the best {\color{OliveGreen}\bf interpretable} model, {\bf boldface} denotes where SPAM Order 3 is best. Runs averaged over 10 random trials with optimal hyperparameters.}
\label{tab:tabular_benchmark_comparison}
\centering
\small
\begin{tabular}{cccccccc}
\hline
\hline 
\multirow{3}{*~}{Model} & {\bf Regression} & {\bf Binary} & \multicolumn{4}{c}{\bf Multi-Class Classification} & {\bf Obj. Det.} \\ 
& RMSE ($\downarrow$) & AUROC ($\uparrow$) & \multicolumn{4}{c}{Accuracy ($\uparrow$)}  & mAP ($\uparrow$) \\ \cline{2-8}
& \multicolumn{1}{c}{CH} & \multicolumn{1}{c}{FICO} & \multicolumn{1}{c}{CovType} & \multicolumn{1}{c}{News} & \multicolumn{1}{c}{CUB} & \multicolumn{1}{c}{iNat} & \multicolumn{1}{c}{CO114}\\ \hline
\multicolumn{8}{c}{ {\color{OliveGreen}\bf Interpretable} Baselines} \\
\hline
Linear (Order 1) & $0.7354^{**}$ & $0.7909^{**}$ & $0.7254^{**}$ & $0.8238^{**}$ & $0.7451^{**}$ & $0.3932^{**}$ & $0.1917^{**}$\\
Linear (Order 2) & $0.7293^{**}$ & $0.7910^{**}$ & $0.7601^{**}$ & --- & $0.7617^{**}$ & $0.4292^{**}$ & $0.2190^{**}$\\
EBMs (Order 1) & $0.5586^{**}$ & $0.7985^{**}$& $0.7392^{**}$& --- & --- & --- & --- \\
EB$^2$Ms (Order 2) & $0.4919^{**}$ & $0.7998^{**}$& --- & --- & --- & --- & --- \\
NAM & $0.5721^{*~}$ & $0.7993^{**}$ & $0.7359^{**}$ & --- & $0.7632^{**}$ & $0.4194^{**}$ & $0.2056^{**}$ \\ \hline
\multicolumn{8}{c}{ {\color{maroon}\bf Uninterpretable} Black-Box Baselines} \\ \hline
% XGBoost  &{\color{maroon}$\mathbf{0.4419^{**}}$} & $0.7266^{**}$ & $0.8863^{**}$ & $0.7677^{**}$ & $0.7186^{**}$ & --- & --- \\ 
XGBoost  &{\color{maroon}$\mathbf{0.4428^{**}}$} & $0.7925^{**}$ & $0.9603^{**}$ & $0.7677^{**}$ & $0.7186^{**}$ & --- & --- \\ 
% DNN & $0.5129^{**}$ & {\color{maroon}$\mathbf{0.7982^{**}}$} & {\color{maroon}$\mathbf{0.9696^{**}}$} & {\color{maroon}$\mathbf{0.8490^{**}}$} & {\color{maroon}$\mathbf{0.7679^{**}}$} & {\color{maroon}$\mathbf{0.4584^{**}}$} & {\color{maroon}$\mathbf{0.2376^{**}}$}\\ \hline
DNN & $0.5014^{**}$ & {\color{maroon}$\mathbf{0.7936^{**}}$} & {\color{maroon}$\mathbf{0.9694^{**}}$} & {\color{maroon}$\mathbf{0.8494^{**}}$} & {\color{maroon}$\mathbf{0.7684^{**}}$} & {\color{maroon}$\mathbf{0.4584^{**}}$} & {\color{maroon}$\mathbf{0.2376^{**}}$}\\ \hline
\multicolumn{8}{c}{ {\color{OliveGreen}\bf Our Interpretable Models} } \\ \hline
SPAM (Linear, Order 2)& $0.6474^{**}$ & $0.7940^{**}$ & $0.7732^{**}$ & {\color{OliveGreen}$\mathbf{0.8472^{**}}$} & {\color{OliveGreen}$\mathbf{0.7786^{**}}$} & $0.4605^{**}$ & {\color{OliveGreen}$\mathbf{0.2361^{**}}$}\\
SPAM (Neural, Order 2)& {\color{OliveGreen}$\mathbf{0.4914^{**}}$} & {\color{OliveGreen}$\mathbf{0.8011^{*~}}$} & {\color{OliveGreen}$\mathbf{0.7770^{**}}$}& --- & $0.7762^{**}$ & {\color{OliveGreen}$\mathbf{0.4689^{**}}$} & ---\\\hline
% \hline\multicolumn{8}{c}{ {\color{maroon}\bf Uninterpretable} Black-Box Baselines} \\ \hline
% XGBoost  &{\color{maroon}$\mathbf{0.4419}$} & $0.7266$ & $0.8863$ & $0.7677$ & $0.7186$ & --- & --- \\ 
% DNN & $0.5129$ & {\color{maroon}$\mathbf{0.7982}$} & {\color{maroon}$\mathbf{0.9696}$} & {\color{maroon}$\mathbf{0.8490}$} & {\color{maroon}$\mathbf{0.7679}$} & {\color{maroon}$\mathbf{0.4584}$} & {\color{maroon}$\mathbf{0.2376}$}\\ \hline
% \multicolumn{8}{c}{ {\color{OliveGreen}\bf Our Interpretable Models} } \\ \hline
% SPAM (Linear, Order 2)& $0.6474$ & $0.7940$ & $0.7732$ & {\color{OliveGreen}$\mathbf{0.8472}$} & {\color{OliveGreen}$\mathbf{0.7786}$} & $0.4605$ & $0.2361$\\
% SPAM (Linear, Order 3)& $0.6410$ & $0.7945$ & $0.8066$ & $\mathbf{0.8520}$ & $0.7741$& {\color{OliveGreen}$\mathbf{0.4684}$} & $0.2368$\\ 
% \hline
% NBM (Order 1) & 
%             $0.5638$  & 
%             {\color{OliveGreen}$\mathbf{0.8048}$}  & 
%             $0.7369$  & 
%             $0.8446$ & 
%             $0.7683$  & 
%             $0.4227$  & 
%         $0.2168$  \\
        
%     NBM (Order 2) & 
%     {\color{OliveGreen}$\mathbf{0.4779}$} & 
%     0.8029 & 
%     {\color{OliveGreen}$\mathbf{0.8908}$}  & 
%     --- & 
%     $0.7770$& 
%     {\color{OliveGreen}$\mathbf{0.4684}$} & 
% {\color{OliveGreen}$\mathbf{0.2378}$}  \\ \hline
SPAM (Linear, Order 3)& $0.6410^{**}$ & $0.7945^{**}$ & $0.8066^{**}$ & $\mathbf{0.8520^{*~}}$ & $0.7741^{**}$& $0.4684^{**}$ & $\mathbf{0.2368^{*~}}$\\ 
SPAM (Neural, Order 3)& $0.4865^{*~}$&  $\mathbf{0.8024^{*~}}$& $0.8857^{**}$& --- & $0.7753^{**}$ & $\mathbf{0.4722^{**}}$ & ---\\ \hline
\hline
\end{tabular}
\end{table}
We select tasks to explore a variety of settings from regression to multi-class classification, and also explore different dataset scales, from a few hundred samples and tens of features to 100K-scale datasets (both in the number of samples and data dimensionality), while ensuring that the features are interpretable. Our datasets are summarized in Table~\ref{tab:tabular_datasets}. Please see Appendix Section~\ref{sec:appendix_dataset_details} for details. For all datasets with no defined train-val-test split, we use a fixed random sample of 70\% of the data for training, 10\% for validation and 20\% for testing. For the 20 Newsgroups dataset, we split the pre-defined training split 7:1 for training and validation, respectively.
\begin{table}[t]
\setlength{\tabcolsep}{1.5pt}
    \centering
    \small
    \caption{Tabular Datasets\label{tab:tabular_datasets}}
    \begin{tabular}{ccccc}
    \hline \hline
        Name & California Housing (CH) & FICO & Cover Type (CovType) & Newsgroups  \\ \hline
        Source & \citet{pace1997sparse} & \citet{fico_community}  & \citet{blackard1999comparative} & \citet{lang1995newsweeder} \\
        Instances & 20,640 & 10,459 & 581,012 & 18,828 \\
        Features & 8 & 23 & 54 & 146,016 \\
        Classes & - & 2 & 7 & 20 \\
        Feature Type & Numeric & Mixed & Mixed & TF-IDF \\ \hline \hline
    \end{tabular}
\end{table}

In an effort to scale interpretable approaches beyond tabular datasets, we consider benchmark problems using the ``Independent Concept Bottleneck'' framework of~\citet{koh2020concept} for image classification and object detection. We use a convolutional neural network (CNN) {\bf backbone} ResNet-50~\citep{he2016deep} that is trained to predict {\em interpretable concepts} (e.g., parts of object) from images. After training the {\bf backbone}, we extract predicted concepts for all inputs, and learn an interpretable classifier {\bf head} from these concepts. In experiments, the backbone remains identical for all comparisons, and we only compare the {\bf head} classifiers (see Appendix Section~\ref{sec:appendix_concept_bottleneck_implementation} for more details). We select three datasets for evaluation in the concept bottleneck setting:
\begin{enumerate}[leftmargin=*,itemsep=0pt,topsep=0pt,parsep=0pt,partopsep=0pt]
    \item {\bf Caltech-UCSD Birds (CUB-200)}~\citep{wah2011caltech}: This is a fine-grained visual categorization dataset where one has to classify between 200 species of birds. The interpretable concepts are 278 {\em binary} bird attributes, e.g., the shape of the beak, the color of the wings, etc. The dataset has 5,994 training and 5,794 validation images. See Appendix Section~\ref{sec:appendix_cub_details} for more details. 
    \item {\bf iNaturalist ``Birds''}~\citep{van2018inaturalist, van2021benchmarking}: iNaturalist can be thought of as a larger version of the previous dataset. We only select the ``Birds'' super-category of samples, which has 414,000 training and 14,860 validation instances across 1,486 classes. Since the iNaturalist dataset does not contain dense part and attribute annotations, we use the {\em predicted} concepts from the CUB-200 backbone model extracted on all samples. 
    \item {\bf Common Objects Dataset} (CO114, Proprietary): Here we consider, for the first time, a concept bottleneck model for object detection. We construct a dataset involving common household objects (e.g., bed, saucer, tables, etc.) with their bounding box annotations. For each bounding box, we collect 2,618 interpretable annotations (e.g., parts, color, etc.). The dataset has 2,645,488 training and 58,525 validation samples across 115 classes with 2,618 interpretable concepts. We report the mean Average Precision (mAP) metric. For more details please refer to Appendix Section~\ref{sec:appendix_w3ig_details}.
\end{enumerate}

Our results are summarized in Table~\ref{tab:tabular_benchmark_comparison}. There are four main takeaways from the results. First, observe that both {\sc SPAM-Linear} and {\sc SPAM-Neural} comfortably outperform their prior interpretable counterparts on all datasets (e.g., Order 2 {\sc SPAM-Linear} outperforms all linear methods -- even the full rank pairwise model), and {\sc SPAM-Neural} comfortably outperforms all non-linear baselines. Next, observe that in all datasets but CoverType, second degree interactions suffice to match or even outperform DNN performance. We will discuss CoverType in detail in the next paragraph. Thirdly, observe that {\sc SPAM} models are as scalable as the black-box approaches, whereas prior work (e.g., NAM and EBMs) are not. In the case of NAM, we were unable to scale due to the sheer number of parameters required to model large datasets, e.g., Newsgroups ($\approx$900M parameters), and for EBMs, the training time and memory requirement increased dramatically for large datasets. Furthermore, EB$^2$Ms do not even support multi-class problems. Finally, observe that for many problems, we do not require {\em non-linear} feature transformations once we model feature interactions: e.g., iNat and CUB.

{\bf CoverType Dataset.} XGBoost and DNNs perform substantially better on CoverType compared to linear or neural SPAM. On analysis, we found that existing SPAM models underfit on CoverType, and hence we increased the total parameters for {\sc SPAM-Neural} via {\em subnets}, identical to NAMs~\citep{agarwal2021neural}, where each feature is mapped to $s$ non-linear features (as opposed to 1 originally). With $s=8$ subnets, the performance of {\sc SPAM-Neural} (order 2) improves to $0.9405$. In comparison, NAMs with $8$ subnets provides a lower accuracy of $0.7551$.

\subsection{Ablation Studies}
\label{sec:ablation}
% We conduct ablation studies to understand the abilities of {\sc SPAM}. Specifically, we first run ablations on the total rank $r$ and degree $k$ of interactions; we explicitly limit the number of higher-order interactions via an $L_1-$sparsity constraint; we test our spectral decay assumption (Assumption~\ref{assumption:singular_value_decay}). 

{\bf Rank and Degree of Interactions}.
\label{sec:ablation_rank_degree}
\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{Images/main_figure.pdf}
    \caption{Ablation of Accuracy with: (A1, A2) Degree $k$; (B1, B2) Rank $r$; (C) $L_1$ Sparsity. \label{fig:ablation_ranks_degree}}
\end{figure}
By Proposition~\ref{prop:approximation}, it is natural to expect the approximation quality to increase with the degree $k$ and rank $r$, i.e., as we introduce more higher-order interactions between features. We ablate the degree $k$ on the tabular benchmark {\bf CoverType} and concept bottleneck benchmark {\bf iNaturalist (Birds)}, as summarized in Figure~\ref{fig:ablation_ranks_degree}{\color{maroon}A}. We observe, as expected, that increasing the degree $k$ leads to moderate improvements beyond $k \geq 3$, but with diminishing returns. Similarly, we examine the effect of the cumulative rank $r$ on performance on the {\bf Newsgroups} and {\bf iNaturalist (Birds)} datasets (Figure~\ref{fig:ablation_ranks_degree}{\color{maroon}B}); we observe that performance is sufficiently insensitive to $r$, and plateaus after a while. We imagine that as $r$ increases, model complexity will dominate and performance will likely begin to decrease, matching the full-rank performance at $r = \cO(d^2)$ for pairwise models.
\paragraph{Sparsity in Higher-Order Relationships.}
A requirement for interpretability is to ensure that the learned models can be explained with a few interpretable concepts. Since the number of higher-order combinations increases with $k$, we examine sparsity to limit the number of active feature assignments. We penalize the objective in Equation~\ref{eqn:optimization_fn} with a regularization term that inhibits dense feature selection. If $\bU = \{\{\bu_{li} \}_{i=1}^{r_l}\}_{l=1}^k$ denotes all the basis vectors in matrix form, we add the penalty $\cR(\btheta) \triangleq \lVert \bU \rVert_1$. This ensures that every basis $\bu$ only captures limited interactions between features, and hence the overall complexity of the model is limited. We examine accuracy as a function of the fraction of non-zero pairwise interactions for a degree 2, rank 800 SPAM on CUB-200 in Figure~\ref{fig:ablation_ranks_degree}{\color{maroon}C}, and find that only $6\%$ of the possible interactions suffice to obtain competitive performance.

\paragraph{Examining Assumption~\ref{assumption:singular_value_decay} (Spectral Decay).} The spectral decay assumption presented in Assumption~\ref{assumption:singular_value_decay} is crucial to obtain reasonable generalization bounds (Theorem~\ref{thm:primary_generalization_bound}). To test this assumption, we examine the spectra of a {\sc SPAM-Linear} (Order 2) model for all 200 of CUB-200 classes. These are depicted in Figure~\ref{fig:amt_results}{\color{maroon}A}. Furthermore, we fit an exponential model on the decay itself, and obtain (in line with Assumption~\ref{assumption:singular_value_decay}) $\gamma = 3$, $C_1 = 0.54$ and $C_2 = 0.006$, all in accordance with the assumption.

==> experiment_details.tex <==
\section{Experimental Details}
\label{sec:appendix_experiment_details}
All our benchmarks are implemented in PyTorch and run on a cluster, where each machine was equipped with $8\times$V100 NVIDIA GPU machines with $32$GB VRAM. We set the batch size of at most $1024$ per GPU, and in case a model is too large to fit a batch size of $1024$, we perform a binary search to find the largest batch size that it will accommodate. All datasets have features renormalized between the range $[0,1]$ for uniformity and simplicity. For all experiments we use the Adam with decoupled weight decay (AdamW) optimizer~\citep{loshchilov2017decoupled}.

\vspace{0.3em}
\subsection{Tabular Dataset Details}
\label{sec:appendix_dataset_details}
We use the following tabular datasets.
\begin{enumerate}[leftmargin=*,itemsep=0pt,topsep=0pt,parsep=0pt,partopsep=0pt]
    \item {\bf California Housing} (CH,~\citet{pace1997sparse}): This dataset was derived from the 1990 U.S. census, and is a regression task, fitting the median house value for California districts using demographic information. The dataset contains 20,640 instances and 8 numeric features. 
    \item {\bf FICO HELOC} (FICO,~\citet{fico_community}): This is a binary task, part of the FICO Explainability challenge. The target variable denotes the ``risk'' of home equity line of credit (HELOC) applicants and features correspond to credit report information. It has 10,459 instances and 23 features.
    \item {\bf Cover Type} (CovType,~\citet{blackard1999comparative}): This multi-class dataset is part of the UCI ML repository~\citep{asuncion2007uci}. The task is classification of forest cover type from cartographic variables. It contains 581,012 instances and 54 attributes over 6 classes.
    \item {\bf 20 Newsgroups} (Newsgroups,~\citet{lang1995newsweeder}): This is a popular benchmark dataset where the problem is multi-class classification of email text into 20 subject categories. Following standard convention, we extract TF-IDF features on the training set, which gives us 18,828 instances and 146,016 features over 20 classes (see Appendix Section~\ref{sec:appendix_newsgroups_dataset} for details).
\end{enumerate}

\vspace{0.3em}
\subsection{20 Newsgroups Feature Extraction}
\label{sec:appendix_newsgroups_dataset}
We use the following feature extraction pipeline from the {\tt sklearn} repository. We first use the {\tt TfIdfVectorizer} to compute the TF-IDF features on only the training set. Next, we transform the testing and validation sets using the learnt vectorizer, and rescale all the features within the range $[0, 1]$. This gives us 18,828 instances and 146,016 features over 20 classes.

\vspace{0.3em}
\subsection{Concept Bottleneck Implementation}
\label{sec:appendix_concept_bottleneck_implementation}
In an effort to scale interpretable approaches to problems beyond tabular datasets, we consider benchmark problems using the ``Sequential Concept Bottleneck'' framework of~\citet{koh2020concept}. The general idea of concept bottleneck (CB) models are to enable feature extraction necessary for problems in domains such as computer vision by learning a black-box model that can first predict human interpretable ``concepts'', and then learn a simple, typically fully-transparent model on these concepts to predict the final category. For example, in the problem of bird species classification from images~\citep{wah2011caltech}, one can consider visible parts and attributes of the birds as intermediary ``concepts'' on which one can learn a linear classifier in order to provide reasonable classification performance while at the same time providing interpretable decisions. Similar approaches have also been explored in the work of, e.g., ~\citet{chen2019looks, ghorbani2019towards} and~\citet{zhang2020invertible}. We consider concept bottleneck models for computer vision tasks. 

\vspace{0.3em}
\subsubsection{CUB-200 Concept Bottleneck}
\label{sec:appendix_cub_details}
The Caltech-UCSD Birds (CUB)-200~\citep{wah2011caltech} dataset is an image classification dataset that has images belonging to 200 different species of birds, a problem that is an instance of the broader problem of {\em fine-grained visual classification}. The dataset is equipped with keypoint annotations of 15 bird parts, e.g., crown, wings, etc., and each part has $\geq 1$ part-attribute labels, e.g., {\em brown leg}, {\em buff neck},  etc. For the concept bottleneck model, we train a convolutional neural network architecture that predicts these intermediary concepts from the images, and then used this trained CNN model (with weights fixed) to extract features that are then trained using one of the several benchmark approaches (including SPAM). One key difference between prior implementations and ours in this concept bottleneck setting is that we ignore laterality within the annotations, e.g., ``left wing'' and ``right wing'' are treated simply as ``wing''.

{\bf CNN architecture}. We train a ResNet-50~\citep{he2016deep} on images resized to the size $448\times 448$ resolution until the last pooling layer of the network ({\tt pool5}). The features are 2048-dimensional but ignoring the spatial pooling, are evaluated on each $14\times 14$ patch within the image. We train part-attribute linear classifiers on these spatially-arranged extracted features, where the part locations are used from the training annotations. Once the network has been trained, we run max-pooling over the $14\times 14$ grid to extract features that are used in the second stage training. Note that this setup is different from the original Concept Bottleneck~\citep{koh2020concept} architecture, as the original setup predicted the keypoints from the entire image, instead of a spatially-supervised version. We use this architecture as the original setup overfit very easily.

\vspace{1.5em}
\subsubsection{Common Objects Dataset Details}
\label{sec:appendix_w3ig_details}
We construct a dataset by collecting public images from Instagram\footnote{\href{https://www.instagram.com}{\ttfamily www.instagram.com}}, involving common household objects (e.g., bed, stove, saucer, tables, etc.) with their bounding box annotations. For each bounding box, we collect 2,618 interpretable annotations, namely, parts (e.g., leg, handle, top, etc.), attributes (e.g., colors, textures, shapes, etc.), and part-attribute compositions. The dataset has 2,645,488 training and 58,525 validation samples across 115 classes with 2,618 interpretable concepts.

\vspace{1.5em}
\subsubsection{Hyperparameters}
\label{sec:appendix_hyperparameters}

Gradient-descent based methods are trained with the Adam with decoupled weight decay (AdamW) optimizer~\cite{loshchilov2017decoupled}. All methods are trained for 1000 epochs on the California Housing and FICO HELOC datasets, 100 epochs on iNaturalist Birds and Common Objects datasets, and 500 epochs on the CoverType, Newsgroups and CUB datasets. We use a cosine annealing learning rate across all gradient-descent based approaches and do a random hyperparameter search within the following specified grids.

\paragraph{Linear (Order 1 and Order 2).}
The learning rate range is $[1\mathrm{e}{-}5, 100]$, and the weight decay interval is $[1\mathrm{e}{-}13, 1.0)$. We use the same interval for $L_1-$regularized models as well.

\paragraph{Deep Neural Networks.}
We experiment with 3 neural network architectures that are all comprised of successive fully-connected layers. The first has 5 hidden layers of the shapes $[128, 128, 64, 64, 64]$ units; the second is three hidden layers deep with $[1024, 512, 512]$ units, and finally we have a shallow but wide architecture having 2 hidden layers with $[2048, 1024]$ units. We report the best accuracies achieved across all three architectures. Moreover, we observed that increasing the depth with more layers did not improve accuracy. 
We search the initial learning rate in the interval $[10^{-6}, 10.0)$, weight decay in  $[1\mathrm{e}{-}9, 1.0)$, dropout in the set $\{0, 0.05, 0.1, 0.2, 0.3, 0.4, 0.5, 0.6, 0.7, 0.8, 0.9\}$.

\paragraph{Neural Additive Models.}
We proceed with the standard proposed architectures in the original implementation of~\citet{agarwal2021neural}. We experiment with two architectures: the first is an MLP with 3 hidden layers and $[64, 64, 32]$ units, and the second is an MLP with 1 hidden layer with $1,024$ units and an ExU activation. We tune the learning rate in the interval $[1\mathrm{e}{-}5, 1.0)$, weight decay in $[1\mathrm{e}{-}9, 1.0)$, output penalty weight in $[1\mathrm{e}{-}{6}, 100)$, dropout and feature dropout in the set $\{0, 0.05, 0.1, 0.2, 0.3, 0.4, 0.5, 0.6, 0.7, 0.8, 0.9\}$.

\paragraph{EBMs.}
We describe the hyperparameter followed by the range of values we search from. 
\begin{itemize}[leftmargin=*,itemsep=0pt,topsep=0pt,parsep=0pt,partopsep=0pt]
    \item Maximum bins: $\{8, 16, 32, 64, 128, 256, 512\}$
    \item Number of interactions: $\{0, 2, 4, 8, 16, 32, 64, 128, 256, 512\}$ ($0$ for EBMs, $\geq 0$ for EB$^2$Ms)
    \item learning rate: $[1\mathrm{e}{-}6, 100)$
    \item maximum rounds: $\{1000, 2000, 4000, 8000, 16000\}$
    \item minimum samples in a leaf node: $\{1, 2, 4, 8, 10, 15, 20, 25, 50\}$
    \item maximum leaves: $\{1, 2, 4, 8, 10, 15, 20, 25, 50\}$
    \item binning: \{``quantile'', ``uniform'', ``quantile\_humanized''\}
    \item inner/outer bags:  $\{1, 2, 4, 8, 16, 32, 64, 128\}$.
\end{itemize}

\paragraph{XGBoost.} 
We describe the hyperparameter followed by the range of values we search from. 
\begin{itemize}[leftmargin=*,itemsep=0pt,topsep=0pt,parsep=0pt,partopsep=0pt]
    \item number of estimators: $\{1, 2, 4, 8, 10, 20, 50, 100, 200, 250, 500, 1000\}$
    \item max-depth: $\{\infty, 2, 5, 10, 20, 25, 50, 100, 2000\}$
    \item $\eta$: $[0.0, 1.0)$
    \item $\lambda$: $[0.0, 1.0)$
    \item $\alpha$: $[0.0, 1.0)$
    \item $\beta$: $[0.0, 1.0)$
    \item {\tt subsample}: $[0.0, 1.0)$
    \item {\tt colsample\_bytree}: $[0.0, 1.0)$
\end{itemize}
\paragraph{CART.}
We describe the hyperparameter followed by the range of values we search from. 
\begin{itemize}[leftmargin=*,itemsep=0pt,topsep=0pt,parsep=0pt,partopsep=0pt]
    \item criterion: \{``absolute error'', ``friedman mse'', ``squared error'', ``poisson''\}
    \item splitter: \{``best'', ``random''\}
    \item minimum samples leaf: $\{4, 8, 16, 32, 64, 128, 256\}$
    \item minimum samples split: $\{4, 8, 16, 32, 64, 128, 256\}$
\end{itemize}

\paragraph{SPAM-Linear}. For SPAM-Linear, there are 4 sets of hyperparameters: initial learning rate (tuned logarithmically from the set $[10^{-7}, 10^2]$), weight decay (tuned logarithmically from the set $[10^{-13}, 10^1]$), dropout for the singular values $\lambda$, which is tuned from the range $[0, 1]$, and the vector of ranks $\br$ which consequently specifies the degree of the polynomial. For degree 2 SPAM, we search ranks from the set $\cS = \{[25], [50], [100], [200], [250], [400], [500], [750], [800], [1000], [1200], [1400], [1600]\}$ and we for order 3, we search from the set $\cS\times\cS$ (i.e., product set of original range).

\paragraph{SPAM-Neural}. For SPAM-Neural, in addition to the 4 original hyperparameters, we search from the NAM space identical to the range employed for NAM (please see above). Regarding the original hyperparameters, we search: initial learning rate (tuned logarithmically from the set $[10^{-7}, 10^2]$), weight decay (tuned logarithmically from the set $[10^{-13}, 10^1]$), dropout for the singular values $\lambda$, which is tuned from the range $[0, 1]$, and the vector of ranks $\br$ which consequently specifies the degree of the polynomial. For degree 2 SPAM, we search ranks from the set $\cS = \{[25], [50], [100], [200], [250], [400], [500], [750], [800], [1000], [1200], [1400], [1600]\}$ and we for order 3, we search from the set $\cS\times\cS$ (i.e., product set of original range).
